Rauzy induction of polygon partitions and toral $\mathbb{Z}^2$-rotations

We extend the notion of Rauzy induction of interval exchange transformations to the case of toral $\mathbb{Z}^2$-rotation, i.e., $\mathbb{Z}^2$-action defined by rotations on a 2-torus. If $\mathcal{X}_{\mathcal{P},R}$ denotes the symbolic dynamical system corresponding to a partition $\mathcal{P}$ and $\mathbb{Z}^2$-action $R$ such that $R$ is Cartesian on a sub-domain $W$, we express the 2-dimensional configurations in $\mathcal{X}_{\mathcal{P},R}$ as the image under a $2$-dimensional morphism (up to a shift) of a configuration in $\mathcal{X}_{\widehat{\mathcal{P}}|_W,\widehat{R}|_W}$ where $\widehat{\mathcal{P}}|_W$ is the induced partition and $\widehat{R}|_W$ is the induced $\mathbb{Z}^2$-action on $W$. We focus on one example $\mathcal{X}_{\mathcal{P}_0,R_0}$ for which we obtain an eventually periodic sequence of 2-dimensional morphisms. We prove that it is the same as the substitutive structure of the minimal subshift $X_0$ of the Jeandel-Rao Wang shift computed in an earlier work by the author. As a consequence, $\mathcal{P}_0$ is a Markov partition for the associated toral $\mathbb{Z}^2$-rotation $R_0$. It also implies that the subshift $X_0$ is uniquely ergodic and is isomorphic to the toral $\mathbb{Z}^2$-rotation $R_0$ which can be seen as a generalization for 2-dimensional subshifts of the relation between Sturmian sequences and irrational rotations on a circle. Batteries included: the algorithms and code to reproduce the proofs are provided.

==> makefile <==
FILE = article4

now:pdf

pdf: image_markov_automorphism.pdf JR_partition.pdf image-walker.pdf SageCreation
	pdflatex $(FILE).tex

bib:
	pdflatex $(FILE).tex
	bibtex $(FILE)
	pdflatex $(FILE).tex
	pdflatex $(FILE).tex

JR_partition.pdf: JR_partition.tex
	pdflatex JR_partition.tex
image_markov_automorphism.pdf: image_markov_automorphism.tex
	pdflatex image_markov_automorphism.tex
image-walker.pdf: image-walker.tex
	pdflatex image-walker.tex

SageCreation:create_images.sage
	 sage create_images.sage

diff:
	latexdiff 2020-05-08-article4.tex article4.tex > diff.tex
	latexdiff 2020-05-08-article4.bbl article4.bbl > diff-bbl.bbl
	latexdiff 2020-05-08-article4-abstract.tex abstract.tex > diff-abstract.tex
	sed -i '/other shortcuts/s/cuts/cuts\n\\input{diff_need_old_macros\.tex}/' diff.tex
	sed -i '/input/s/abstract/diff-abstract/' diff.tex
	sed -i '/\\bibliography/s/\\bibliography{\.\.\/biblio}/\\input{diff-bbl\.bbl}/' diff.tex
	- pdflatex -interaction=nonstopmode diff.tex
	#bibtex diff
	- pdflatex -interaction=nonstopmode diff.tex
	- pdflatex -interaction=nonstopmode diff.tex

answers:
	rst2pdf answers_to_review.txt answers_to_review.pdf

arxiv:bib
	tar -cvzf 2021-12-01-article4-arxiv.tar.gz \
	article4.tex \
	article4.bbl \
	abstract.tex \
	create_images.sage \
	makefile \
	SageCreation/JR_beta_0.tex \
	SageCreation/JR_beta_2.tex \
	SageCreation/JR_beta_3.tex \
	SageCreation/JR_beta_4.tex \
	SageCreation/JR_beta_5.tex \
	SageCreation/JR_beta_6.tex \
	SageCreation/JR_beta_7.tex \
	SageCreation/JR_beta_8.tex \
	SageCreation/JR_beta_9.tex \
	SageCreation/JR_perm8to10.tex \
	SageCreation/JR_selfP8.tex \
	SageCreation/JR_selfPU.tex \
	image-walker.pdf \
	image_markov_automorphism.pdf \
	JR_partition.pdf \
	SageCreation/partition_JR_P1.pdf \
	SageCreation/partition_JR_P3.pdf \
	SageCreation/partition_JR_P4.pdf \
	SageCreation/partition_JR_P5.pdf \
	SageCreation/partition_JR_P5_scaled.pdf \
	SageCreation/partition_JR_P6.pdf \
	SageCreation/partition_JR_P7.pdf \
	SageCreation/partition_JR_P7_scaled.pdf \
	SageCreation/partition_JR_P8.pdf \
	SageCreation/partition_JR_P9.pdf \
	SageCreation/partition_JR_P9_scaled.pdf \
	SageCreation/partition_JR_P10.pdf \
	SageCreation/partition_PU.pdf

tar:bib
	#sudo pip3 install arxiv-collector
	#arxiv-collector article4.tex --dest 2021-01-06-article4-arxiv-collector.tar.gz
	#arxiv-collector article4.tex --dest 2021-08-10-article4-arxiv-collector.tar.gz
	arxiv-collector article4.tex --dest 2021-09-30-article4-arxiv-collector.tar.gz

.PHONY : clean
clean :
	rm -f $(FILE).aux $(FILE).log
	rm -f $(FILE).blg $(FILE).bbl
	rm -f $(FILE).tdo $(FILE).out
	rm -f $(FILE).toc $(FILE).dvi
	#rm -f $(FILE).py $(FILE).sage $(FILE).sout
	rm -f $(FILE).pdf
	rm -rf SageCreation
	rm -f image-walker.pdf
	rm -f image-walker.log
	rm -f image-walker.aux
	rm -f image_markov_automorphism.pdf
	rm -f image_markov_automorphism.aux
	rm -f image_markov_automorphism.log
	rm -f JR_partition.pdf
	rm -f JR_partition.log
	rm -f JR_partition.aux
	rm -f create_images.sage.py




